A Unified Framework for Hopsets and Spanners

Given an undirected graph $G=(V,E)$, an {\em $(\alpha,\beta)$-spanner} $H=(V,E')$ is a subgraph that approximately preserves distances; for every $u,v\in V$, $d_H(u,v)\le \alpha\cdot d_G(u,v)+\beta$. An $(\alpha,\beta)$-hopset is a graph $H=(V,E")$, so that adding its edges to $G$ guarantees every pair has an $\alpha$-approximate shortest path that has at most $\beta$ edges (hops), that is, $d_G(u,v)\le d_{G\cup H}^{(\beta)}(u,v)\le \alpha\cdot d_G(u,v)$. Given the usefulness of spanners and hopsets for fundamental algorithmic tasks, several different algorithms and techniques were developed for their construction, for various regimes of the stretch parameter $\alpha$. In this work we develop a single algorithm that can attain all state-of-the-art spanners and hopsets for general graphs, by choosing the appropriate input parameters. In fact, in some cases it also improves upon the previous best results. We also show a lower bound on our algorithm. In \cite{BP20}, given a parameter $k$, a $(O(k^{\epsilon}),O(k^{1-\epsilon}))$-hopset of size $\tilde{O}(n^{1+1/k})$ was shown for any $n$-vertex graph and parameter $0<\epsilon<1$, and they asked whether this result is best possible. We resolve this open problem, showing that any $(\alpha,\beta)$-hopset of size $O(n^{1+1/k})$ must have $\alpha\cdot \beta\ge\Omega(k)$.

==> LIPICS/latexmac.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   PAGE LENGTH PARAMETERS
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Springer Verlag format: depends on font size. For 12pt:
% 9.2 x 6.3 inches, which is roughly 23 x 15.8 cm
% Latest - in cm, and slightly changed: 23.8 x 15.4cm (narrower).
%
% MENTION: REDUCE TO 83%
%
%Margins adjusted properly
\def\svformat{
\setlength{\textheight}{23.8cm}
\setlength{\textwidth}{15.4cm}
\setlength{\evensidemargin}{0in}
\setlength{\oddsidemargin}{0in}
\setlength{\headsep}{10pt}
\setlength{\topmargin}{-0.3in}
\setlength{\columnsep}{0.375in}
\setlength{\itemsep}{0pt}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Springer Verlag format: depends on font size. For 10pt:
%
% PROBLEM - wisdom does not have 10pt.sty
%
% For 10pt they wanted pages of 5.3 x 7.9 inches.
% But apparently they changed that: Now, they specify things in cm,
% and require 12.8 x 19.8 cm (which is 5.1 x 7.9 inches) (narrower).
%Margins not adjusted properly
\def\svtenformat{
\setlength{\textheight}{19.8cm}
\setlength{\textwidth}{12.8cm}
\setlength{\evensidemargin}{0.4in}
\setlength{\oddsidemargin}{0.4in}
\setlength{\headsep}{10pt}
\setlength{\topmargin}{0.2in}
\setlength{\columnsep}{0.375in}
\setlength{\itemsep}{0pt}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Dense format
\def\denseformat{
\setlength{\textheight}{9in}
\setlength{\textwidth}{6.9in}
\setlength{\evensidemargin}{-0.2in}
\setlength{\oddsidemargin}{-0.2in}
\setlength{\headsep}{10pt}
\setlength{\topmargin}{-0.3in}
\setlength{\columnsep}{0.375in}
\setlength{\itemsep}{0pt}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New Dense format
\def\newdenseformat{
\setlength{\textheight}{8.9in}
\setlength{\textwidth}{6.6in}
\setlength{\evensidemargin}{-0.2in}
\setlength{\oddsidemargin}{-0.2in}
\setlength{\headsep}{10pt}
\setlength{\topmargin}{-0.3in}
\setlength{\columnsep}{0.375in}
\setlength{\itemsep}{0pt}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mid format
\def\midformat{
\setlength{\textheight}{8.9in}
\setlength{\textwidth}{6.7in}
\setlength{\evensidemargin}{-0.19in}
\setlength{\oddsidemargin}{-0.19in}
\setlength{\headheight}{0in}
\setlength{\headsep}{10pt}
\setlength{\topsep}{0in}
\setlength{\topmargin}{0.0in}
\setlength{\itemsep}{0in}       % 10pt is too big with the 1.2 stretch
\renewcommand{\baselinestretch}{1.1}
\parskip=0.06in
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mid-spacy format
\def\midspacyformat{
\setlength{\textheight}{8.9in}
\setlength{\textwidth}{6.7in}
\setlength{\evensidemargin}{-0.19in}
\setlength{\oddsidemargin}{-0.19in}
\setlength{\headheight}{0in}
\setlength{\headsep}{10pt}
\setlength{\topsep}{0in}
\setlength{\topmargin}{0.0in}
\setlength{\itemsep}{0in}       % 10pt is too big with the 1.2 stretch
\renewcommand{\baselinestretch}{1.2}
\parskip=0.070in
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Spacy format
\def\spacyformat{
\setlength{\textheight}{8.8in}
\setlength{\textwidth}{6.5in}
\setlength{\evensidemargin}{-0.18in}
\setlength{\oddsidemargin}{-0.18in}
\setlength{\headheight}{0in}
\setlength{\headsep}{10pt}
\setlength{\topsep}{0in}
\setlength{\topmargin}{0.0in}
\setlength{\itemsep}{0in}      % 10pt is too big with the 1.2 stretch
\renewcommand{\baselinestretch}{1.2}
\parskip=0.080in
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Super spacy format
\def\superspacyformat{
\setlength{\textheight}{8in}
\setlength{\textwidth}{5.7in}
\setlength{\evensidemargin}{0.2in}
\setlength{\oddsidemargin}{0.2in}
\setlength{\headheight}{0in}
\setlength{\headsep}{20pt}
\setlength{\topsep}{0in}
\setlength{\topmargin}{0.0in}
\setlength{\itemsep}{0in}      % 10pt is too big with the 1.2 stretch
\renewcommand{\baselinestretch}{1.2}
\parskip=0.080in
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% DEFINING THEOREM-LIKE ENVIRONMENTS 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Examine sometime. 
% Here: the first, theorem, is defined [section], 
%       and the rest are defined [theorem].
%
% Possible: define all as [section].
%
% Better, if I copy just a few lines.
%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
%\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{comment}[theorem]{Comment}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{property}[theorem]{Property}
\newtheorem{dfn}[theorem]{Definition}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\weizprinter{\setlength{\topmargin}{0.3in}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% MY MACROS
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\nipar{\par\noindent}
\def\xskip#1{$\mbox{\hskip #1}$}
\def\yskip#1{$\vbox{\vskip #1}$}
\def\boldhead#1:{\par\vskip 7pt\noindent{\bf #1:}\hskip 10pt}
\def\ithead#1:{\par\vskip 7pt\noindent{\it #1:}\hskip 10pt}
\def\ceil#1{\lceil #1\rceil}
\def\floor#1{\lfloor #1\rfloor}
\def\inline#1:{\par\vskip 7pt\noindent{\bf #1:}\hskip 10pt}
\def\midinline#1:{\par\noindent{\bf #1:}\hskip 10pt}
\def\dnsinline#1:{\par\vskip -7pt\noindent{\bf #1:}\hskip 10pt}
\def\ddnsinline#1:{\newline{\bf #1:}\hskip 10pt}
\def\largeinline#1:{\par\vskip 7pt\noindent{\large\bf #1:}\hskip 10pt}
%
%The next command is essentially equivalent to \section*,
%except smaller font
\def\heading#1{\par\medskip\noindent{\bf #1}\par\smallskip\noindent}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\comment #1\commentend{}
\long\def\commhide #1\commhideend{}
\long\def\commfull #1\commend{#1}
\long\def\commabs #1\commenda{}
\long\def\commtim #1\commendt{#1}
\long\def\commb #1\commbend{}
%
%% FOR LN:
%
\long\def\commedit #1\commeditend{} % Editing comments, marked also by $>>>$ 

\long\def\commB #1\commBend{}       % Omit in 1996 (both TR and Siena)
                                    % Leave for phase B.

\long\def\commex #1\commexend{}     % LN home exercise (hide solutions)

\long\def\commsiena #1\commsienaend{}  % omit in Siena, show in TR
                                         
\long\def\commBI #1\commBIend{}  % omit in Bar-Ilan
                                         
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\long\def\CProof #1\CQED{}
\def\qed{\mbox{}\hfill $\Box$\\}
\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def\QED{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
\def\inQED{\quad\quad\blackslug}
\def\Qed{\QED}
\def\QUAD{$\Box$}

%\def\Proof{\noindent{\bf Proof:~}}
\def\Proof{\par\noindent{\bf Proof:~}}
\def\Proofb{\par\noindent\hbox{hskip 7pt}{\bf Proof:~}}
\def\proof{\Proof}
\def\Sketch{\par\noindent{\bf Proof Sketch:~}}
\def\sketch{\Sketch}
\def\Method{\noindent{\bf Proof Method}: }
\long\def\PPP#1{\noindent{\bf Proof:}{ #1}{\quad\blackslug\lower 8.5pt\null}}
\long\def\PP#1{\noindent {\bf Proof}:{ #1} $\Box$ \\}
\long\def\P#1{{\Proof}{#1}\Qed\\}
\def\Remark{\noindent{\bf Remark:~}}
\def\Comment{\noindent{\bf Comment:~}}
\long\def\denspar #1\densend
{#1}
%{{\renewcommand{\baselinestretch}{0.8}\small #1\par\medskip}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  DELIMITER PAIRS AND MATHEMATICAL FUNCTIONS
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\attention}[1]{{\bf \textcolor{red}{\# #1 \#}} \\}

\newcommand{\pare}[1]{\left( #1\right)}
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\norm}[1]{\parallel #1\parallel}
\newcommand{\card}[1]{\left| #1\right|}
\newcommand{\bigo}[1]{O\left( #1\right)}
\newcommand{\ang}[1]{\left\langle #1 \right\rangle}
%\newcommand{\prob}[1]{\Pr\left\{ #1 \right\}}

\newcommand{\OO}[1]{O\left( #1\right)}
\newcommand{\OM}[1]{\Omega\left( #1 \right)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  MARGINAL NOTES FOR COMMUNICATING WITH COAUTHORS
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\marginparwidth}{1in}
\setlength{\marginparpush}{-5ex}
\newif\ifnotesw\noteswtrue% T to show box & marginal notes; F supresses.
\newenvironment{change}%
   {\ifnotesw\marginpar[\hfill\(\top\)]{\(\top\)}\fi}%
   {\ifnotesw\marginpar[\hfill\(\bot\)]{\(\bot\)}\fi}
\newcommand{\deletion}{\ifnotesw\marginpar[\hfill\(\vartheta\)]{\
(\vartheta\)}\fi}
\newcommand{\mnote}[1]%
    {\ifnotesw\marginpar%
        [{\scriptsize\it\begin{minipage}[t]{\marginparwidth}
        \raggedleft#1%
                        \end{minipage}}]%
        {\scriptsize\it\begin{minipage}[t]{\marginparwidth}
        \raggedright#1%
                        \end{minipage}}%
    \fi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% SPECIAL LETTERS
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}
%%%%%%%%%%%%%%%%%%
\def\hA{{\hat A}}
\def\hB{{\hat B}}
\def\hC{{\hat C}}
\def\hD{{\hat D}}
\def\hE{{\hat E}}
\def\hF{{\hat F}}
\def\hG{{\hat G}}
\def\hH{{\hat H}}
\def\hI{{\hat I}}
\def\hJ{{\hat J}}
\def\hK{{\hat K}}
\def\hL{{\hat L}}
\def\hM{{\hat M}}
\def\hN{{\hat N}}
\def\hO{{\hat O}}
\def\hP{{\hat P}}
\def\hQ{{\hat Q}}
\def\hR{{\hat R}}
\def\hS{{\hat S}}
\def\hT{{\hat T}}
\def\hU{{\hat U}}
\def\hV{{\hat V}}
\def\hW{{\hat W}}
\def\hX{{\hat X}}
\def\hY{{\hat Y}}
\def\hZ{{\hat Z}}
\def\hb{{\hat b}}
\def\hGamma{{\hat \Gamma}}
\def\hPi{{\hat \Pi}}
\def\htau{{\hat \tau}}
\def\hgamma{{\hat \gamma}}
\def\hi{{\hat i}}
\def\hj{{\hat j}}
%\def\wmax{{\hat \omega}}
%%%%%%%%%%%%%%%%%%
\def\bA{{\bar A}}
\def\bB{{\bar B}}
\def\bC{{\bar C}}
\def\bD{{\bar D}}
\def\bE{{\bar E}}
\def\bF{{\bar F}}
\def\bG{{\bar G}}
\def\bH{{\bar H}}
\def\bI{{\bar I}}
\def\bJ{{\bar J}}
\def\bK{{\bar K}}
\def\bL{{\bar L}}
\def\bM{{\bar M}}
\def\bN{{\bar N}}
\def\bO{{\bar O}}
\def\bP{{\bar P}}
\def\bQ{{\bar Q}}
\def\bR{{\bar R}}
\def\bS{{\bar S}}
\def\bT{{\bar T}}
\def\bU{{\bar U}}
\def\bV{{\bar V}}
\def\bW{{\bar W}}
\def\bX{{\bar X}}
\def\bY{{\bar Y}}
\def\bZ{{\bar Z}}
\def\bff{{\bar f}}      % seems that \bf is occupied
\def\bq{{\bar q}}
\def\bx{{\bar x}}
\def\btau{{\bar \tau}}
\def\bomega{{\bar \omega}}
%%%%%%%%%%%%%%%%%%
\def\tA{{\tilde A}}
\def\tB{{\tilde B}}
\def\tC{{\tilde C}}
\def\tD{{\tilde D}}
\def\tE{{\tilde E}}
\def\tF{{\tilde F}}
\def\tG{{\tilde G}}
\def\tH{{\tilde H}}
\def\tI{{\tilde I}}
\def\tJ{{\tilde J}}
\def\tK{{\tilde K}}
\def\tL{{\tilde L}}
\def\tM{{\tilde M}}
\def\tN{{\tilde N}}
\def\tO{{\tilde O}}
\def\tP{{\tilde P}}
\def\tQ{{\tilde Q}}
\def\tR{{\tilde R}}
\def\tS{{\tilde S}}
\def\tT{{\tilde T}}
\def\tU{{\tilde U}}
\def\tV{{\tilde V}}
\def\tW{{\tilde W}}
\def\tX{{\tilde X}}
\def\tY{{\tilde Y}}
\def\tZ{{\tilde Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\dist{{\mathit{dist}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% DOUBLING LETTERS (e.g. IE as E).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For the Z I changes to san-serif, to avoid strange tags,
% and decreased the spacing (from -3 to -4).
%
\def\MathF{\hbox{\rm I\kern-2pt F}}
\def\MathP{\hbox{\rm I\kern-2pt P}}
\def\MathR{\hbox{\rm I\kern-2pt R}}
\def\MathZ{\hbox{\sf Z\kern-4pt Z}}
\def\MathN{\hbox{\rm I\kern-2pt I\kern-3.1pt N}}
\def\MathC{\hbox{\rm \kern0.7pt\raise0.8pt\hbox{\footnotesize I}
\kern-4.2pt C}}
\def\MathQ{\hbox{\rm I\kern-6pt Q}}

%% Fails:
%% \def\MathC{\hbox{\rm \kern0.7pt\raise0.8pt\hbox{\specialeightrm I}
%% \kern-4.2pt C}}
\def\MathE{\hbox{{\rm I}\hskip -2pt {\rm E}}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ANOTHER NICE FONT TO USE - for doubled letters

\def\dblA{\Bbb{A}}
\def\dblM{\Bbb{M}}
\def\dblN{\Bbb{N}}
\def\dblP{\Bbb{P}}
\def\dblR{\Bbb{R}}
\def\dblW{\Bbb{W}}
\def\dblZ{\Bbb{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% MATHEMATICAL NOTATION
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \tends  -  for limit notation (f(x)--->0)
% Avishai's version:::
\newcommand{\Tends}[1]
   {\mathrel{\mathop{\longrightarrow}\limits_{#1\to\infty}}}
% Malki's version:::
\newsavebox{\ttop}\newsavebox{\bbot}
\newcommand{\tends}[4]{\sbox{\ttop}{${#1}\longrightarrow{#2}$}
\savebox{\bbot}[1\wd\ttop]{\hfill$\scriptstyle{#3}\rightarrow{#4}$\hfill}
\rlap{\usebox{\ttop}}\raisebox{-7pt}{\usebox{\bbot}}\; }
%
\def\mod{\pmod}
% nice AMS TeX empty set
\newcommand{\emp}{\varnothing}
\def\eps{\epsilon}
\def\epsi{\varepsilon}
\def\polylog{\mbox{polylog}}
\def\poly{\mbox{poly}}
\def\setmns{\setminus}
\def\scrpolylog{\mbox{\rm\scriptsize polylog~}}
%\def\polylog{\mbox{polylog}\,}
%\def\polylog{\mbox{\it polylog}\,}
\newcommand{\half}{{1\over2}}
\def\st{\mbox{~~s.t.~~}}
\def\nin{{~\not \in~}}
\def\emset{\emptyset}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% PROBABILITY TERMINOLOGY
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\Prob}[1]{\Pr\left( #1 \right)}
\newcommand{\Exp}[1]{\MathE\left( #1 \right)}
%\newcommand{\Set}[1]{\left\{ #1 \right\}}
%\def\Prob{\mbox{\tt Prob}}
\def\Event{\cE}
%\def\Expect{\mbox{\bf E}}
\newcommand{\Prob}{\MathP}
\newcommand{\Expect}{\MathE}

%%%###########################################################


\def\etal{\emph{et~al.}}
\def\Erdos{Erd\H{o}s}  
\def\Szemeredi{Szemer\'edi}
\def\Toth{T\'{o}th}		% Geza
\def\Turan{Tur\'an}
